Shape Optimization using the Finite Element Method on Multiple Meshes

An important step in shape optimization with partial differential equation constraints is to adapt the geometry during each optimization iteration. Common strategies are to employ mesh-deformation or re-meshing, where one or the other typically lacks robustness or is computationally expensive. This paper proposes a different approach, in which the computational domain is represented by multiple, independent meshes. A Nitsche based finite element method is used to weakly enforce continuity over the non-matching mesh interfaces. The optimization is preformed using an iterative gradient method, in which the shape-sensitivities are obtained by employing the Hadamard formulas and the adjoint approach. An optimize-then-discretize approach is chosen due to its independence of the FEM framework. Since the individual meshes may be moved freely, re-meshing or mesh deformations can be entirely avoided in cases where the geometry changes consists of rigid motions or scaling. By this free movement, we obtain robust and computational cheap mesh adaptation for optimization problems even for large domain changes. For general geometry changes, the method can be combined with mesh-deformation or re-meshing techniques to reduce the amount of deformation required. We demonstrate the capabilities of the method on several examples, including the optimal placement of heat emitting wires in a cable to minimize the chance of overheating, the drag minimization in Stokes flow, and the orientation of 25 objects in a Stokes flow.

==> error_eikonal.tex <==
\begin{table}[h]\centering\begin{tabular}{|c|c|c|}
 \hline $\alpha$& $J(\Gamma_2^{k}-\alpha Dn)-J(\Omega^k)- \mathrm{d} J(\Omega^k)[-\alpha Dn]$ & Rate \\ 
\hline 5.000e-05 & 7.801e+00  & - \\
\hline 2.500e-05 & 2.205e+00 & 1.823e+00\\
\hline 1.250e-05 & 5.947e-01 & 1.891e+00\\
\hline 6.250e-06 & 1.592e-01 & 1.901e+00\\
\hline 3.125e-06 & 4.366e-02 & 1.867e+00\\
\hline 1.563e-06 & 1.266e-02 & 1.786e+00\\
\hline 7.813e-07 & 4.014e-03 & 1.657e+00\\
\hline 3.906e-07 & 1.425e-03 & 1.494e+00\\
\hline 1.953e-07 & 5.670e-04 & 1.330e+00\\
\hline 9.766e-08 & 2.470e-04 & 1.199e+00\\
\hline \end{tabular}\caption{Error-rates for finite difference gradient compared with analytic gradient}\label{tab:error_eikonal}\end{table}


==> table3_config.tex <==
\begin{table}[h]\begin{tabular}{|c|c|c|c|c|}
\hline \multicolumn{5}{|c|}{\textbf{MultiMesh}}\\
 \hline Mesh size & $L^2$-error in control & $L^2$-error in state & Rate & \# Iterations \\ 
\hline 0.059 & 1.749e-02 & 6.813e-05 & - & 121 \\
\hline 0.030 & 4.783e-03 & 1.792e-05 & 1.955 & 119 \\
\hline 0.015 & 1.250e-03 & 4.625e-06 & 1.980 & 134 \\
\hline 0.008 & 3.316e-04 & 1.224e-06 & 1.981 & 133 \\
\hline 0.004 & 8.164e-05 & 2.975e-07 & 1.989 & 145 \\
\hline \multicolumn{5}{|c|}{\textbf{Single mesh}}\\
 \hline Mesh size & $L^2$-error in control & $L^2$-error in state & Rate & \# Iterations \\
\hline 0.062 & 1.953e-02 & 7.994e-05 & - & 111 \\
\hline 0.031 & 5.231e-03 & 1.942e-05 & 1.901 & 118 \\
\hline 0.016 & 1.336e-03 & 4.828e-06 & 1.969 & 137 \\
\hline 0.008 & 3.355e-04 & 1.206e-06 & 1.993 & 142 \\
\hline 0.004 & 8.489e-05 & 3.016e-07 & 1.983 & 137 \\
\hline \end{tabular}\caption{Errors and convergence rate for the Poisson optimization problem. Comparison between MultiMesh and the same mesh described as a single mesh.}\label{convgoptcg}\end{table}

